Channel-Attentive Graph Neural Networks

Graph Neural Networks (GNNs) set the state-of-the-art in representation learning for graph-structured data. They are used in many domains, from online social networks to complex molecules. Most GNNs leverage the message-passing paradigm and achieve strong performances on various tasks. However, the message-passing mechanism used in most models suffers from over-smoothing as a GNN's depth increases. The over-smoothing degrades GNN's performance due to the increased similarity between the representations of unrelated nodes. This study proposes an adaptive channel-wise message-passing approach to alleviate the over-smoothing. The proposed model, Channel-Attentive GNN, learns how to attend to neighboring nodes and their feature channels. Thus, much diverse information can be transferred between nodes during message-passing. Experiments with widely used benchmark datasets show that the proposed model is more resistant to over-smoothing than baselines and achieves state-of-the-art performances for various graphs with strong heterophily. Our code is at https://github.com/ALLab-Boun/CHAT-GNN.

==> components/benchmark_reported.tex <==
\begin{table}[t!]
\centering
\caption{Comparison with the best performances reported by AERO-GNN~\cite{aero} and Ordered GNN~\cite{gonn} studies.}
\begin{tabular}{llll}
\toprule
 & AERO-GNN & Ordered GNN & \textbf{CHAT-GNN} \\
\midrule
chameleon & $\underline{71.6 \pm 2.4}$ & $\mathbf{72.3 \pm 2.3}$ & $70.5 \pm 2.1$ \\
squirrel & $61.8 \pm 2.4$ & $\underline{62.4 \pm 2.0}$ & $\mathbf{64.3 \pm 1.5}$ \\
cornell & $\underline{81.2 \pm 6.8}$ & $\mathbf{87.0 \pm 4.7}$ & $72.2 \pm 4.2$ \\
actor & $\underline{36.6 \pm 1.1}$ & $\mathbf{38.0 \pm 1.0}$ & $35.6 \pm 1.3$ \\
texas & $\underline{84.3 \pm 5.2}$ & $\mathbf{86.2 \pm 4.1}$ & $\underline{84.3 \pm 5.4}$ \\
wisconsin & $84.8 \pm 3.3$ & $\mathbf{88.0 \pm 3.7}$ & $\underline{87.3 \pm 3.2}$ \\
\bottomrule
\end{tabular}
\label{tab:benchmark_reported}
\end{table}

==> components/best_hyp.tex <==
\begin{table*}[]
    \centering
    \caption{Best hyperparameters of CHAT-GNN for each benchmark dataset.}
    \begin{tabular}{ll}
    \toprule
    dataset & best hyperparameters \\
    \midrule
    roman-empire & lr=0.005, layer\_norm=True, num\_layers=6, hidden\_size=256, weight\_decay=0.0005, post\_transform=True \\
    amazon-ratings & lr=0.005, layer\_norm=True, num\_layers=5, hidden\_size=512, weight\_decay=0.0001, post\_transform=False \\
    minesweeper & lr=0.01, layer\_norm=True, num\_layers=10, hidden\_size=128, weight\_decay=0.0005, post\_transform=False \\
    tolokers & lr=0.005, layer\_norm=True, num\_layers=6, hidden\_size=64, weight\_decay=0.0001, post\_transform=True \\
    questions & lr=0.01, layer\_norm=True, num\_layers=8, hidden\_size=256, weight\_decay=0.0005, post\_transform=False \\
    chameleon & lr=0.005, layer\_norm=True, num\_layers=16, hidden\_size=128, weight\_decay=0.0005, post\_transform=False \\
    squirrel & lr=0.005, layer\_norm=True, num\_layers=13, hidden\_size=256, weight\_decay=0.0005, post\_transform=False \\
    cornell & lr=0.01, layer\_norm=False, num\_layers=4, hidden\_size=128, weight\_decay=0.0005, post\_transform=False \\
    actor & lr=0.005, layer\_norm=False, num\_layers=8, hidden\_size=32, weight\_decay=0.0005, post\_transform=True \\
    texas & lr=0.01, layer\_norm=True, num\_layers=2, hidden\_size=256, weight\_decay=0.0001, post\_transform=False \\
    wisconsin & lr=0.005, layer\_norm=False, num\_layers=3, hidden\_size=256, weight\_decay=0.0001, post\_transform=False \\
    cora & lr=0.01, layer\_norm=False, num\_layers=5, hidden\_size=64, weight\_decay=0.0005, post\_transform=False \\
    citeseer & lr=0.005, layer\_norm=False, num\_layers=3, hidden\_size=64, weight\_decay=0.0005, post\_transform=False \\
    pubmed & lr=0.01, layer\_norm=False, num\_layers=2, hidden\_size=64, weight\_decay=0.0001, post\_transform=True \\
    \bottomrule
    \end{tabular}
    \label{tab:best_hyp}
\end{table*}

==> components/best_layer.tex <==
\begin{table}[t!]
    \centering
    \caption{Best performing layer of our model on each benchmark dataset.}
    \begin{tabular}{lrl}
    \toprule
    \textbf{dataset} & \textbf{best layer} & \textbf{search space} \\
    \midrule
    roman-empire & 10 & \{2, 4, 6, 8, 10, 12\} \\
    amazon-ratings & 6 & \{2, 3, 4, 5, 6\} \\
    minesweeper & 14 & \{2, 4, 6, 8, 10, 12, 14\} \\
    tolokers & 10 & \{2, 3, 4, 5, 6, 7, 8, 9, 10\} \\
    questions & 10 & \{2, 4, 6, 8, 10, 12\} \\
    chameleon & 12 & \{2, 4, 6, 8, 10, 12, 14, 16, 18\} \\
    squirrel & 12 & \{2, 4, 6, 8, 10, 11, 12, 13, 14\} \\
    cornell & 2 & \{2, 4, 6, 8, 10\} \\
    actor & 8 & \{2, 4, 6, 8\} \\
    wisconsin & 2 & \{2, 3, 4, 5\} \\
    cora & 5 & \{2, 3, 4, 5\} \\
    citeseer & 4 & \{2, 3, 4, 5\} \\
    pubmed & 2 & \{2, 3, 4, 5\} \\
    \bottomrule
    \end{tabular}
    \label{tab:best_layer}
\end{table}

==> components/heatmap_single.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/chatgnn_minesweeper_att_vecs_heatmap_single.pdf}
    \caption{Cosine similarity between $\beta_{ji}$'s for a randomly selected node $i$ throughout the message-passing layers of CHAT-GNN. The plot illustrates how the node $i$ sends different messages based on specific neighbors and layers.}
    \label{fig:heatmap_single}
\end{figure}

==> components/heatmaps_more.tex <==
% \begin{figure*}[t]
%   \parbox{\linewidth}{
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/chatgnn_minesweeper_att_vecs_heatmap.pdf}
%   }
%   \caption{Visualization of pairwise cosine similarities of channel attention vectors at deeper layers for Minesweeper dataset.}
%   \label{fig:heatmap_more_1}
% \end{figure*}
% \begin{figure*}[t!]
%   \parbox{\linewidth}{
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/chatgnn_roman-empire_att_vecs_heatmap.pdf}
%   }
%   \caption{Visualization of pairwise cosine similarities of channel attention vectors at deeper layers for Roman-Empire dataset.}
%   \label{fig:heatmap_more_2}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/chatgnn_minesweeper_att_vecs_heatmap.pdf}
  \caption{Visualization of pairwise cosine similarities of channel attention vectors at deeper layers for Minesweeper dataset.}
  \label{fig:heatmap_more_1}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/chatgnn_roman-empire_att_vecs_heatmap.pdf}
  \caption{Visualization of pairwise cosine similarities of channel attention vectors at deeper layers for Roman-Empire dataset.}
  \label{fig:heatmap_more_2}
\end{figure*}

\begin{figure*}[t]
  \parbox{0.49\linewidth}{
    \centering
    \includegraphics[width=\linewidth]{images/chatgnn_pubmed_att_vecs_heatmap.pdf}
  }
  \parbox{0.49\linewidth}{
    \centering
    \includegraphics[width=\linewidth]{images/chatgnn_wisconsin_att_vecs_heatmap.pdf}
  }
  \caption{Visualization of pairwise cosine similarities of channel attention vectors at deeper layers for Pubmed and Wisconsin datasets.}
  \label{fig:heatmap_more_3}
\end{figure*}

==> sections/acknowledgments.tex <==
\begin{acks}
    Acknowledgments
\end{acks}

==> sections/theory.tex <==
\section{Theoretical Analysis}
In this section, we discuss the effectiveness of channel-attentive message-passing by providing some theoretical findings. We start with the notion of local smoothness. \textit{Local variation} of node $v$ according to graph signal $\mathbf{X}$ is defined as follows \cite{emerging_gsp}:
\begin{equation}
    \mathcal{E}_v(\mathbf{X}) = \sum_{w \in \mathcal{N}(v)} \| \mathbf{x}_v - \mathbf{x}_w \|^2
\end{equation}
Then, the \textit{Dirichlet Energy} is defined as the sum of local variations across all nodes, which can be seen as a measure of global smoothness \cite{emerging_gsp, graphcon}:
\begin{equation}
    \mathcal{E}(\mathbf{X}) = \frac{1}{N} \sum_{v \in \mathcal{V}} \mathcal{E}_v(\mathbf{X})
    \label{eq:dirichlet}
\end{equation}
Thus, the global smoothness of the node features depends on the local variations. The following proposition indicates that the change in the local variation between consecutive GNN layers is bounded by the distance between the aggregated messages.

\begin{proposition}
    Let us assume that we have a GNN in which the (k+1)-th layer's update is as follows: $\mathbf{h}_v^{(k+1)} = \mathbf{h}_v^{(k)} + \mathbf{m}_v^{(k+1)}$, where $\mathbf{m}_v^{(k+1)}$ is the output of a message-passing layer. Then, the change in the local variation of node $v$, $\Delta_{(k+1)} \mathcal{E}_v = \mathcal{E}_v^{(k+1)} - \mathcal{E}_v^{(k)}$ satisfies the following inequality:
    \begin{equation}
        \Delta_{(k+1)} \mathcal{E}_v \leq \sum_{w \in \mathcal{N}(v)} (\delta_{wv}^{(k+1)})^2 + 2c\delta_{wv}^{(k+1)}
    \end{equation}
    where $\delta_{wv}^{(k+1)} = \| \mathbf{m}_w^{(k+1)} - \mathbf{m}_v^{(k+1)} \|$ and $c = \max \| \mathbf{h}_w^{(k)} - \mathbf{h}_v^{(k)} \|$.

\label{prop1}
\end{proposition}
\begin{IEEEproof}
\begin{IEEEeqnarray}{lCl}
\Delta_{(k+1)} \mathcal{E}_v &=& \sum_{w \in \mathcal{N}(v)} 
\Big ( \| \mathbf{h}_w^{(k)} + \mathbf{m}_w^{(k+1)} - 
(\mathbf{h}_v^{(k)} + \mathbf{m}_v^{(k+1)}) \|^2\IEEEnonumber\\
&&- \| \mathbf{h}_w^{(k)} - \mathbf{h}_v^{(k)} \|^2 \Big )\IEEEnonumber\\
&=& \sum_{w \in \mathcal{N}(v)} \Big [ \Big ( 
    \| \mathbf{h}_w^{(k)} + \mathbf{m}_w^{(k+1)} - 
(\mathbf{h}_v^{(k)} + \mathbf{m}_v^{(k+1)}) \| \IEEEnonumber\\
&&- \| \mathbf{h}_w^{(k)} - \mathbf{h}_v^{(k)} \|
\Big )\Big ( 
    \| \mathbf{h}_w^{(k)} + \mathbf{m}_w^{(k+1)} - \IEEEnonumber\\
&&(\mathbf{h}_v^{(k)} + \mathbf{m}_v^{(k+1)}) \|  + \| \mathbf{h}_w^{(k)} - \mathbf{h}_v^{(k)} \|
\Big )   \Big ]
\end{IEEEeqnarray}

Using the triangle inequality, we get:
\begin{IEEEeqnarray}{lCl}
\Delta_{(k+1)} \mathcal{E}_v &\leq& \sum_{w \in \mathcal{N}(v)} 
\Big [ \Big ( 
    \| \mathbf{m}_w^{(k+1)} - \mathbf{m}_v^{(k+1)} \|
\Big )\IEEEnonumber\\
&&\Big ( 
    \| \mathbf{m}_w^{(k+1)} - \mathbf{m}_v^{(k+1)} \| 
    + 2\| \mathbf{h}_w^{(k)} - \mathbf{h}_v^{(k)} \|
\Big )   \Big ]\IEEEnonumber\\
&=& \sum_{w \in \mathcal{N}(v)} (\delta_{wv}^{(k+1)})^2 + 2c\delta_{wv}^{(k+1)}
\end{IEEEeqnarray}
\end{IEEEproof}

Proposition~\ref{prop1} shows that the upper bound on the change in the local variation is determined by how different the message vectors of neighboring nodes are. The over-smoothing effect begins when a GNN layer's output for a node is similar to its neighbors. Next, we present another proposition that compares the standard graph attention and our proposed channel-wise graph attention in terms of how likely the $\delta_{wv} = \| \mathbf{m}_w - \mathbf{m}_v \|$  would be non-zero.


\begin{proposition}
    Assume that we have a pair of nodes $v$ and $w$ that satisfy $\mathcal{N}(v) = \mathcal{N}(w)$, and positive node features $\mathbf{X}$. Further, assume that message vectors with standard and channel-wise attention are calculated as $\mathbf{m}_v =  \sum_{k \in \mathcal{N}(v)} \alpha_{vk} \mathbf{x}_k $ and $\mathbf{m}_v' = \sum_{k \in \mathcal{N}(v)} \beta_{vk} \odot \mathbf{x}_k  $, respectively. Lastly, we assume that each unnormalized attention score $\alpha_{vk}$ and $\beta_{vkd}$ are all independent random variables. Then, we have the following inequalities satisfied:
    \begin{equation}
        \Pr(\delta_{m_{vw}}^* > 0 ) \leq | \mathcal{N}(v) | P^*
    \end{equation}
    \begin{equation}
        \Pr(\delta_{m_{vw}'}^* > 0 ) \leq | \mathcal{N}(v) | D P^*
    \end{equation}
    where $\delta_{m_{vw}}^* = \sum_{k \in \mathcal{N}(v)} |\alpha_{vk} - \alpha_{wk}| \| \mathbf{x}_k \|$ and $\delta_{m_{vw}'}^* = \sum_{k \in \mathcal{N}(v)} \| (\beta_{vk} - \beta_{wk}) \odot \mathbf{x}_k \|$ are the respective upper bounds of $\delta_{vw}$ under the standard and channel-wise attention settings, $D$ is the dimensionality of feature vectors and channel-wise attention vector $\beta$, and $P^*$ is the maximum possible value that $\Pr( | \alpha - \alpha' | > 0 )$ can attain for two arbitrary attention scores $\alpha$ and $\alpha'$. 

\label{prop2}
\end{proposition}
\begin{IEEEproof}
    We begin with the first inequality. We can see that $\delta_{m_{vw}}^*$ is greater than zero if for at least one neighbor $k$, we have $|\alpha_{vk} - \alpha_{wk}| \neq 0$. Therefore, using Boole's inequality, we have the following:
    \begin{IEEEeqnarray}{lCl}
        \Pr(\delta_{m_{vw}}^* > 0 ) &=& \Pr( \bigcup_{k \in \mathcal{N}(v)} \{  |\alpha_{vk} - \alpha_{wk}| \neq 0 \} ) \IEEEnonumber\\
        &\leq& \sum_{k \in \mathcal{N}(v)} \Pr(|\alpha_{vk} - \alpha_{wk}| \neq 0)\IEEEnonumber\\
        &\leq& | \mathcal{N}(v) | P^*
    \end{IEEEeqnarray}

    Now, we prove the second equality. Similarly, we see that the $\delta_{m_{vw}'}^*$ is greater than zero if for at least one dimension $d$ for one neighbor $k$, we have $|\beta_{vkd} - \beta_{wkd}| \neq 0$. Again, we utilize Boole's inequality as follows:
    \begin{IEEEeqnarray}{lCl}
        \Pr(\delta_{m_{vw}'}^* > 0 ) &=& \Pr( \bigcup_{k \in \mathcal{N}(v)} \{  \| \beta_{vk} - \beta_{wk} \| \neq 0 \} ) \IEEEnonumber\\
        &\leq& \sum_{k \in \mathcal{N}(v)} \Pr(\| \beta_{vk} - \beta_{wk} \| \neq 0 )\IEEEnonumber\\
        &=& \sum_{k \in \mathcal{N}(v)} \Pr( \bigcup_{d=1}^D \{  | \beta_{vkd} - \beta_{wkd} | \neq 0 \} ) \IEEEnonumber\\
        &\leq& \sum_{k \in \mathcal{N}(v)} \sum_{d=1}^D \Pr(   | \beta_{vkd} - \beta_{wkd} | \neq 0  )\IEEEnonumber\\
        &\leq& | \mathcal{N}(v) | D P^*
    \end{IEEEeqnarray}
\end{IEEEproof}

Therefore, in the worst case where two nodes $v$ and $w$ have exactly the same neighborhood, the channel-attentive attention mechanism is more likely to avoid collapsed message vectors. The following sections present the experimental setup and results on well-known benchmark datasets. 
